Probing supermassive black hole seed scenarios with gravitational wave measurements

The process whereby the supermassive black holes populating the centers of galaxies have been assembled remains to be established, with the relative importance of seeds provided by collapsed Population-III stars, black holes formed in nuclear star clusters via repeated mergers, or direct collapses of protogalactic disks yet to be determined. In this paper we study the prospects for casting light on this issue by future measurements of gravitational waves emitted during the inspirals and mergers of pairs of intermediate-mass black holes, discussing in particular the roles of prospective measurements by LISA and the proposed atom interferometers AION and AEDGE. We find that, the expected number of detectable IMBH binaries is $O(100)$ for LISA and AEDGE and $O(10)$ for AION in low-mass seeds scenarios and goes down to $O(10)$ for LISA and below one for AEDGE and AION in high-mass seed scenarios. This allows all of these observatories to probe the parameters of the seed model, in particular if at least a fraction of the SMBHs arise from a low-mass seed population. We also show that the measurement accuracy of the binary parameters is, in general, best for AEDGE that sees very precisely the merger of the binary.

==> reply.tex <==
This paper performs novel exploratory tests to assess the ability of
different gravitational wave detectors to distinguish black hole seeding
models. Newly proposed atom interferometer experiments, AION and AEDGE,
are considered. This paper is very clear in its methodology and likely
to be helpful for motivating these missions. My comments on the
manuscript are minor.

1. Throughout, the authors should make sure to use \citep{} as
appropriate; most citations are provided with only the year in
parentheses.

2. The paper would benefit from a paragraph in the introduction
comparing and contrasting these three missions as well as PTA. It may
not be obvious to the general reader that they are sensitive to
different frequencies and therefore different masses and merger stages.

3. There are two ways in which I believe the estimates of the number of
observable binaries should be considered optimistic upper limits. Since
this paper has the goal of demonstrating seeding constraints using these
instruments at all, I do not believe it to be strictly necessary to
alter calculations based on these comments, but there should at least be
some cautionary discussion about these assumptions.

3a. The authors should emphasize for the reader that they are assuming
that the halo merger rate is equal to the black hole merger rate (times
$p_BH$). That is, additional delays related to binary formation and
evolution following a halo merger are not accounted for. When estimating
LISA event rates, modeling these delays cause orders of magnitude in
spread among theoretical estimates (see recent review by Amaro-Seoane et
al. 2023). This may be especially problematic for the black hole mass
range considered here, since black holes may have a more difficult time
sinking to the centers of dwarf galaxies (e.g., Reines et al. 2020,
Bellovary et al. 2021)

3b. The authors use a black hole mass to the stellar mass relation obtained
for ellipticals and classical bulges, but the conclusions of this paper
are most sensitive to low-mass black holes in low-mass galaxies. The
more appropriate relationship from Reines and Volonteri (2015) would be
equation 4, which is systematically lower by over an order of magnitude.
Note, for example, that in Figure 1 a Milky Way mass halo of $10^12$ solar
masses is assigned a black hole over $10^8$ solar masses. The authors
should also double-check the claimed observed scatter of sigma=1.1. On
the one hand, this is a larger value than claimed in Reines and
Volonteri equation 6, and on the other hand, this appears smaller than
the spread visible in Figure 1.


We thank the referee for the positive feedback and suggestions to improve the paper. The changes in the draft are marked in red, please find below our responses to the enumerated comments:

1. We have now fixed the citation issue by using \citep{} in most of the places.

2. We have extended the 4th paragraph in the introduction to include the relevant frequency and mass ranges.

3. We have added a new paragraph at the end of Sec. 2 to emphasize the uncertainties in the merger rate estimate and a new footnote 2 about the stellar mass-BH mass relation. One objective of this paper was to extend the merger rate of SMBH that the NANOgrav background needs to lower masses. The AGN relation found by Reines and Volonteri (2015) doesn't fit the background, although we have also extended the discussion around it. For the mass of Sgr A, note that the virial mass of the Milky Way is not very well known currently. For example, $2*10^11\, M_{\odot}$ was obtained recently using the Gaia data (arXiv:2309.00048). This indicates that the Sgr A mass is consistent with the mass relation we use. For the scatter of sigma=1.1, notice that we use the lognormal distribution, Eq. (2). So, 0.47dex corresponds to sigma = ln($10^0.47$) = 1.1. We have added a footnote to clarify this. Also, we thank the referee for noticing that this scatter wasn't correct in Fig. 1. We have now fixed that and checked that it was correct in the other computations.


